Self-Assembly of Shapes at Constant Scale using Repulsive Forces

The algorithmic self-assembly of shapes has been considered in several models of self-assembly. For the problem of \emph{shape construction}, we consider an extended version of the Two-Handed Tile Assembly Model (2HAM), which contains positive (attractive) and negative (repulsive) interactions. As a result, portions of an assembly can become unstable and detach. In this model, we utilize fuel-efficient computation to perform Turing machine simulations for the construction of the shape. In this paper, we show how an arbitrary shape can be constructed using an asymptotically optimal number of distinct tile types (based on the shape's Kolmogorov complexity). We achieve this at $O(1)$ scale factor in this straightforward model, whereas all previous results with sublinear scale factors utilize powerful self-assembly models containing features such as staging, tile deletion, chemical reaction networks, and tile activation/deactivation. Furthermore, the computation and construction in our result only creates constant-size garbage assemblies as a byproduct of assembling the shape.

==> ConstructionGadgets/gadgets.tex <==
This construction uses pre-constructed assemblies called gadgets. These gadgets are designed to work in a temperature $\tau = 10$ system. In our figures, a perpendicular black line through the middle of the edge of two adjacent tiles indicates a unique infinite strength bond (i.e. the strength of the glue is $\gg$ than $\tau$ such that no detachment events can occur in which these tiles are separated). Each gadget provides a different function to the shape creation process. Some gadgets have special-case versions which are very similar to their standard counterparts. For clarity of understanding, in this section we will only be describing the standard version of each gadget. For a description of all special case gadgets, see Appendix~\ref{app:specialgadgets}.

%Tape
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.28\textwidth}
		\includegraphics[scale=3.9]{ConstructionGadgets/tape_1.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{.6\textwidth}
		\includegraphics[scale=3.9]{ConstructionGadgets/tape_2.pdf}
		\caption{}
	\end{subfigure}\\
	\begin{subfigure}[b]{1\textwidth}
		\centering
		\includegraphics[scale=2.4]{ConstructionGadgets/tape_3.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) A single section of a fuel-efficient Turing machine \emph{tape} used in this construction, along with buffer tiles that separate tape sections. (b) A series of joined tape sections. (c) A completed \emph{tape} consisting of all \emph{forward} instructions.}
	\label{fig:tapesections}
\end{figure}
 \textbf{Turing Machine Tape.}
A detailed look at a fuel-efficient Turing machine \emph{tape} is seen in Figure~\ref{fig:tapesections}. Notice each tape section has a pair of tiles on top of it where the information is stored. When talking about the \emph{tape} from Section~\ref{sec:overview}.2, each pair of dark grey tiles on top of the tape sections represents a piece of information describing the \emph{path}.

%overlay
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/overlay_gadget.pdf}
		\caption{Overlay Gadget}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/overlay_helpers.pdf}
		\caption{Overlay Helpers}
	\end{subfigure}
	\caption{(a) The overlay gadget comes in two parts, and attaches to the tape using its \emph{h}-type glues, which are unique to the end of a completed Turing machine tape. (b) Four filler blocks make up the overlay helpers. Three of these helpers are standard fillers, but the horizontal domino piece has multiple versions to cover the different information bits on the tape.}
	\label{fig:overlaygadget}
\end{figure}

%combined figures
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/read_combined.pdf}
		\caption{Read gadget and helpers}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/walking_combined.pdf}
		\caption{Walk gadget and helpers}
	\end{subfigure}
	\caption{(a) The read gadget (dark grey) has as many versions as the tape has different types of instructions. The \emph{F} glues in this figure indicate that this gadget reads the \emph{forward} instruction. The negative \emph{Q} glue is used for detaching the gadget once the tape is read. The read helpers (blue) allow the first information block (green) to attach to the top of the overlay, which essentially extracts the info from the tape. (b) Like the read gadget, the walking gadget (dark grey) has versions specific to the different information types. The \emph{F} glues indicate that this walker will be walking an \emph{F}-type instruction down the path. The negative \emph{D} glue allows the gadget to be detached once the information block has walked one step. The light-green assembly is the corresponding information block. The two other helpers (olive drab) remove the previous info block/helpers and the walking gadget.}
	\label{fig:combinedgadgets1}
\end{figure}

\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/extension_combined.pdf}
		\caption{Extension gadget and helpers}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=4.0]{ConstructionGadgets/reduction_combined.pdf}
		\caption{Reduction gadget and helpers}
	\end{subfigure}
	\caption{(a) The path extension gadget (dark grey) also has information-specific versions. The glue in the third topmost position (\emph{F} in this figure) determines which version of the gadget attaches. The \emph{X} glue allows the first portions of the new path piece to attach. The \emph{V} glues are utilized by the extension helpers. The light grey assemblies attach piece-by-piece to form a path portion. The purple helpers are used to detach the extension gadget, along with the info block that allowed this extension. (b) The tape reduction gadget (dark grey) attaches using its \emph{A2} and \emph{U} glues, who's counterparts are only exposed if a given \emph{tape} section has already been read. All other glues on the gadget are used by its helpers. The reduction helpers (red and dark grey) attach to the gadget, and the negative \emph{o} glue is responsible for the destabilization of the gadget, along with the previously read tape section.}
	\label{fig:combinedgadgets2}
\end{figure}

 \textbf{Overlay Gadget.}
The overlay gadget (Fig~\ref{fig:overlaygadget}) is the first assembly to attach to the completed \emph{tape}, and allows the attachment of subsequent assemblies (overlay helpers) which end up covering the entire \emph{tape}. This is the overlay process described in Section~\ref{sec:overview}.2. Each bit of information on the \emph{tape} has a corresponding overlay piece that will attach to it. This step essentially ``flattens'' the surface of the \emph{tape}, making the information easily readable by the gadgets used in this construction. In addition to being designed to initiate the overlay process, the overlay gadget also has glues on its east side which will be the starting location for the \emph{path} we are constructing. The \emph{path} will grow off of the \emph{tape}.

 \textbf{Read Gadgets.}
The read gadget (Fig~\ref{fig:combinedgadgets1}a) is required for ``reading'' the Turing machine \emph{tape} (discussed in Sec~\ref{sec:overview}.2). Essentially, this gadget extracts the information that is relayed from the \emph{tape} through the overlay blocks. It can only attach to the leftmost tape section if it has not previously been read. Once attached, the gadget allows the attachment of an information block (corresponding to the information being read) that will be used to carry the build instructions through the rest of our construction. The read gadget was designed to produce this information block, alter the \emph{tape} section that is being read (making it unreadable), and then detach from the assembly. This design ensures that each \emph{tape} section is only read once, and allows us to transfer the instructions to other locations in our construction via the walking gadgets.

 \textbf{Walking Gadgets.}
The walking gadgets (Fig~\ref{fig:combinedgadgets1}b) begin the information walking process (Sec~\ref{sec:overview}.2) which allows instructions to travel throughout our construction. Once the information block has attached and the read gadget is removed, the walking gadgets can get to work. These gadgets work by attaching to an information block, placing another copy of that block in front of it, and removing the previous block, thus moving the information block forward one ``step". The walking gadget is detached after the new information block is placed. This process is repeated until the information has traveled to the end of the \emph{path}, at which point it is used to construct the next \emph{path} portion. This method is desirable because it does not allow duplicate readable instructions to be attached to the path at any time.

 \textbf{Path Extension Gadgets.}
Once the information block is at the end of the \emph{path}, a path extension gadget (Figure~\ref{fig:combinedgadgets2}a) can attach to the assembly. Once attached, the gadget allows the \emph{path} extension process (Sec~\ref{sec:overview}.2) to begin, which extends the \emph{path} in a given direction (forward, left, or right) based on the instruction carried by the information block. We designed this gadget to essentially replace an instruction block with a corresponding \emph{path} portion. This design allows us to attach a $O(1)$ sized \emph{path} portion for each instruction read from the \emph{tape}.

 \textbf{Tape Reduction Gadget.}
The tape reduction gadget (Fig~\ref{fig:combinedgadgets2}b) initiates the tape reduction process mentioned in Section~\ref{sec:overview}.2. This gadget attaches to a previously read \emph{tape} section and removes it, allowing the next section to be read. This technique is desirable because it allows us to break apart the \emph{tape} into $O(1)$ sized pieces as we use it. As the \emph{tape} is reduced, the \emph{path} continues to grow until there are no more \emph{tape} sections to be read.

==> Introduction/stuffToCite.tex <==
\subsection{Stuff to Cite}

Kolmogorov Optimal shapes at high scale, aTAM:
\cite{SolWin07}

Kolmogorov Optimal shapes at log scale in RNA staged model:
\cite{RNAPods}

Kolmogorov Optimal shapes, constant scale, CRN-TAM model:
\cite{Schiefer2015}

Negative glue tiles in 3D simulating 2D signal passing:
\cite{Fochtman2015}

Negatives glues 2HAM, fuel-efficient computation:
\cite{SS2013FEC}

Negative glues aTAM, temperature 1 computation
\cite{rgTAM}

Negative glues aTAM, space efficient computation
\cite{DotKarMas10}

Negative glues 2HAM, temperature 1, computation
\cite{PRS2016RMN}




==> LineConstruction/line_construction.tex <==
In this section, we detail the steps presented in the construction overview (Sec~\ref{sec:overview}.2). This is the process by which information is read from the \emph{tape} and portions of the \emph{path} are assembled. For clarity, in this section we will just be showing how \emph{forward} instructions are read in order to build a linear section of the \emph{path}. Although each glue strength can be found in the figure captions, there is a full table of glue strengths in Table~\ref{tbl:gluetable}.

\input{Tables/gluestrength.tex}

%Overlay
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_overlay_1.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_overlay_2.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_overlay_3.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) The Overlay Initiator Gadget attaches to the end of the tape ($t1 + $ \textit{h\^} $ = 8 + 2 \geq \tau = 10$), and then an overlay tile, unique to the end of the tape, attaches ($h + h\ast + i1 = 2 + 3 + 5 \geq \tau$). This begins the rest of the overlay process. Two vertical domino assemblies attach ($q2 + i2 = 5 + 5 \geq \tau, q1 + i3 = 5 + 5 \geq \tau $), and finish covering the first tape section as seen in (b). A 2x3 overlay block attaches ($q3 + w + e = 5 + 2 + 3 \geq \tau$), and covers the first portion of the next tape section. At this point, one of three horizontal domino overlay assemblies attach depending on which information bit is on the tape section. In (c), since the $f$ bit is on the tape, it's corresponding overlay domino attaches ($f + f\ast + i1 = 2 + 3 + 5 \geq \tau $) which carries the \textit{forward} instruction. Two more vertical dominos finish covering the tape section, and this process is repeated until every section of the tape is covered.}
	\label{fig:lineoverlay}
\end{figure}

\textbf{Overlay.}
The Overlay Initiator Gadget attaches to the end of the completed \emph{tape}, and begins the overlay process (Fig \ref{fig:lineoverlay}). Each bit of information on the tape is covered by a corresponding overlay section, allowing the information to be read on top of the overlay. This process continues, section by section, until the entire tape is covered. Once finished, the overlay layer will act as an interface, allowing the gadgets discussed in Section~\ref{sec:gadgets} to use the information on the \emph{tape}.

%Read
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_1.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_2.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_3.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_4.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_5.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_read_6.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) The Read Gadget attaches ($n + T + F = 2 + 7 + 1 \geq \tau$). (b) This allows the first read-helpers to attach ($K + M = 9 + 1 \geq \tau, J1 + A1 = 8 + 2 \geq \tau$). In (c) the first form of an information block attaches ($F + F + J2 = 1 + 1 + 8 \geq \tau$). Since the \textit{forward} version of the read gadget was used, the \textit{forward} information block is placed. After the information block is placed, the penultimate read-helper attaches ($A2 + A2 + O1 = 2 + 2 +7 \geq \tau$). (d) The final read-helper attaches ($J3 + J3 + Q = 8 + 8 - 4 \geq \tau$). Notice the attraction of the $J3$ glues overcomes the negativity of the $Q$ glue, allowing attachment. This, however, destabilizes the read gadget along the cut shown in (e)($F + F + M + n + T + F + Q = 1 + 1 + 1 + 2 + 7 + 1 - 7 \leq \tau$). (f) The unstable gadget falls off and the information block (by way of the read-helpers) remains attached to the tape-overlay.}
	\label{fig:lineread}
\end{figure}

\textbf{Read.}
The Read Gadget attaches to the leftmost section of the overlaid tape (Fig \ref{fig:lineread}), only if it has not been read before. The read-helpers begin attaching and allow for the corresponding information block to attach as well. Now, the information that was on this \emph{tape} section is contained in separate block. Once the information block is present, the remaining read-helpers can attach. The final helper destabilizes the read gadget, allowing it to fall off and expose the newly attached information block. Notice, that after the read gadget detaches, the overlay is now altered and this \emph{tape} section can no longer be read.

%Walk
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_1.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_2.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_3.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_4.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_5.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_walk_a_6.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) A Walking Gadget (specific to the information block) attaches to the overlay and the information block ($F + F + +J1 = 1 + 1 + 8 \geq \tau$). (b) A new \textit{forward} information block attaches ($F + O2 + X = 1 + 7 + 2 \geq \tau$). The first walking-helper attaches to the new information block and the overlay($J1 + Z1 + D = 8 + 9 - 7 \geq \tau$). (c) The negative interaction between the $D$ glues destabilizes the old information block, along with the two walking-helpers($J2 + A2 + A2 + F + F + D = 8 + 2 + 2 + 1 + 1 - 7 \leq \tau$). (d) The old information block and walking-helpers break off, and the second walking-helper now ($Z2 + Z2 + D = 9 + 9 - 7 \geq \tau$). (e) Once the second walking-helper is attached, the walking gadget becomes unstable ($F + O2 + J1 + D = 1 + 7 + 8 - 7 \leq \tau$). (f) The walking gadget detaches and leaves the new information block with two walking-helpers attached.}
	\label{fig:linewalk1}
\end{figure}

\textbf{Information Walking.}
The information block only allows the correct walking gadget to attach and begin the walking process (Fig \ref{fig:linewalk1}). Once attached, the walking gadget allows a new information block (of the same type) to attach, while also detaching the the previous info block. Notice that this detachment will always be a $O(1)$ size. After the previous information is removed, the walking gadget detaches as well, allowing the new info block to interact with other gadgets. Thus, the same information has traveled from the \emph{tape}, through the overlay, and is now traveling along the \emph{tape}.

%Extend
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_1.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_2.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_3.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_4.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_5.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=1.75]{LineConstruction/line_extend_a_6.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) The forward-extension gadget attaches to the information block and Turing tape ($B + C + F + p = 3 + 4 + 1 + 2 \geq \tau$). (b) Once the gadget it in place, two path blocks attach ($X + H1 = 2 + 8 \geq \tau, P2 + H2 = 2 + 8 \geq \tau$). (c) The extension-helpers attach. The first ($O3 + V1 = 7 + 9 \geq \tau$), and the second ($V0 + V0 = 9 + 9 \geq \tau$).(d) The second extension-helper comes with the negative $D$ glue that causes targeted destabilization ($X + p + J1 + X + D = 2 + 2 + 8 + 2 - 7 \leq \tau$). The extension gadget and its helpers, along with the information block and its helpers are no longer stable along their tape-overlay edges. (e) Once the unstable assemblies detach, a second half of the path piece attaches ($P2 + P2 = 9 + 9 \geq \tau$). (f) The final result is a one path-pixel extension of the path.}
	\label{fig:lineextend}
\end{figure}

\textbf{Path Extension.}
Once the information block has walked as far as it can, the information is finally used to extend the path (Fig \ref{fig:lineextend}). The path can extend in one of three directions (\textit{forward}, \textit{left}, or \textit{right}), depending on which information block is being read. The extension gadget reads the information block, extends the path in the given direction, and then detaches all but the newly extended path. Notice that the path is extended by a $O(1)$ size, and a $O(1)$ size detachment occurs. One $4x4$ \emph{path} portion is $\frac{1}{36}^{th}$ of a pixel of the shape.

%Reduction
\begin{figure}[]
	\centering
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_1.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_2.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_3.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_4.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_5.pdf}
		\caption{}
	\end{subfigure}
	$\quad$
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\includegraphics[scale=2.0]{LineConstruction/line_reduction_6.pdf}
		\caption{}
	\end{subfigure}
	\caption{(a) The tape reduction gadget attaches to the read-helpers ($A2 + U = 2 + 8 \geq \tau$). (b) The first reduction helpers attach ($u1 + u3 = 8 + 8 \geq \tau, u2 + u4 = 8 + 8 \geq \tau$). (c) Filler tiles attach ($s + s = 8 + 8 \geq \tau$), and create a strong bond to the tape reduction gadget. (d) Two final reduction helpers attach ($s + m + o = 8 + 8 - 5 \geq \tau$). (e) The two negative \textit{o} glues cause a strong targeted destabilization of the previously read tape section ($e + u1 + u2 + o + o = 3 + 8 + 8 - 5 - 5 \leq \tau$). (f) The tape reduction gadget detaches with the used tape section, allowing the next section of the tape to be read.}
	\label{fig:linereduce}
\end{figure}

\textbf{Tape Reduction.}
After a tape section has been read, we no longer need it. Instead of continuing to grow the assembly, we choose to remove $O(1)$ size portions of the \emph{tape} as it is being read. Because of the attachments left behind from the read/walk processes, the tape reduction gadget can attach to the tape section that was read (Fig \ref{fig:linereduce}). The gadget then removes itself, along with the previously read tape section, exposing the next section of the tape for reading. 
